Measurement of the leptonic asymmetry in ttbar events produced in ppbar collisions at sqrt(s)=1.96 TeV

We measure the asymmetry in the charge-weighted rapidity of the lepton in semileptonic ttbar decays recorded with the CDF II detector using the full Tevatron Run II sample, corresponding to an integrated luminosity of 9.4/fb. A parametrization of the asymmetry as a function of the charge-weighted rapidity is used to correct for the finite acceptance of the detector and recover the production-level asymmetry. The result of afb(lep) = 0.094 +0.032 -0.029 is to be compared to the standard model next-to-leading-order prediction of afb(lep) = 0.038 +-0.003.

==> tables/AfblepResultSummaryInclusive.tex <==
\begin{tabular}{cr@{$\pm$}lc}
\hline
\hline
Correction level       & \multicolumn{2}{c}{CDF Data}                               & {\sc powheg} \\
\hline
Data Only              & $0.067$ & $0.016$             & $0.031$ \\
Backgrounds Subtracted & $0.070$ & $0.019 \pm 0.012$ & $0.022$ \\
Fully Extrapolated     & $0.094$ & $0.024^{+0.022}_{-0.018}$ & $0.027$ \\
\hline
\hline
\end{tabular}


==> tables/LabFrameAfbqYhad.tex <==
\begin{tabular}{cccccc}
\hline
\hline
Sample & $N_{data}$ & $N_{background}$ & $N_{signal}$ & Data Asymmetry & Signal Asymmetry \\
\hline
Inclusive    & $2653$ & $529.3$ & $2123.7$ & $-0.049 \pm 0.019$ &  $-0.075 \pm 0.022$ \\
\hline
Electrons    & $1209$ & $262.9$ & $946.1$ & $-0.050 \pm 0.029$ &  $-0.078 \pm 0.032$ \\
Muons        & $1444$ & $266.4$ & $1177.6$ & $-0.048 \pm 0.026$ &  $-0.073 \pm 0.029$ \\
\hline
4 Jet        & $1946$ & $434.1$ & $1511.9$ & $-0.060 \pm 0.023$ &  $-0.096 \pm 0.026$ \\
5 Jet        & $ 707$ & $95.2$ & $611.8$ & $-0.021 \pm 0.038$ &  $-0.025 \pm 0.040$ \\
\hline
Positive     & $1278$ & $265.2$ & $1012.8$ & $-0.069 \pm 0.028$ &  $-0.096 \pm 0.031$ \\
Negative     & $1375$ & $264.1$ & $1110.9$ & $-0.031 \pm 0.027$ &  $-0.057 \pm 0.030$ \\
\hline
\end{tabular}


==> tables/LabFrameAfbqYlep.tex <==
\begin{tabular}{cccccc}
\hline
\hline
Sample & $N_{data}$ & $N_{background}$ & $N_{signal}$ & Data Asymmetry & Signal Asymmetry \\
\hline
Inclusive    & $2653$ & $529.3$ & $2123.7$ & $+0.053 \pm 0.019$ &  $+0.056 \pm 0.022$ \\
\hline
Electrons    & $1209$ & $262.9$ & $946.1$ & $+0.029 \pm 0.029$ &  $+0.028 \pm 0.032$ \\
Muons        & $1444$ & $266.4$ & $1177.6$ & $+0.073 \pm 0.026$ &  $+0.079 \pm 0.029$ \\
\hline
4 Jet        & $1946$ & $434.1$ & $1511.9$ & $+0.063 \pm 0.023$ &  $+0.070 \pm 0.026$ \\
5 Jet        & $ 707$ & $95.2$ & $611.8$ & $+0.027 \pm 0.038$ &  $+0.023 \pm 0.040$ \\
\hline
Positive     & $1278$ & $265.2$ & $1012.8$ & $+0.050 \pm 0.028$ &  $+0.059 \pm 0.031$ \\
Negative     & $1375$ & $264.1$ & $1110.9$ & $+0.056 \pm 0.027$ &  $+0.054 \pm 0.030$ \\
\hline
\end{tabular}

